Comparative Analysis of Deepfake Detection Models: New Approaches and Perspectives

The growing threat posed by deepfake videos, capable of manipulating realities and disseminating misinformation, drives the urgent need for effective detection methods. This work investigates and compares different approaches for identifying deepfakes, focusing on the GenConViT model and its performance relative to other architectures present in the DeepfakeBenchmark. To contextualize the research, the social and legal impacts of deepfakes are addressed, as well as the technical fundamentals of their creation and detection, including digital image processing, machine learning, and artificial neural networks, with emphasis on Convolutional Neural Networks (CNNs), Generative Adversarial Networks (GANs), and Transformers. The performance evaluation of the models was conducted using relevant metrics and new datasets established in the literature, such as WildDeep-fake and DeepSpeak, aiming to identify the most effective tools in the battle against misinformation and media manipulation. The obtained results indicated that GenConViT, after fine-tuning, exhibited superior performance in terms of accuracy (93.82%) and generalization capacity, surpassing other architectures in the DeepfakeBenchmark on the DeepSpeak dataset. This study contributes to the advancement of deepfake detection techniques, offering contributions to the development of more robust and effective solutions against the dissemination of false information.

==> elempostextuais/anexA.tex <==
\chapter{Título deste anexo}
\label{anexoA}


==> elempostextuais/anexB.tex <==
\chapter{Título do ANEXO B}
\label{anexoB}


==> elempostextuais/apenA.tex <==
\chapter{Inclusão de Código-fonte}
\label{apendiceA}

Por enquanto os código estão presentes em um \href{https://colab.research.google.com/drive/1qIqNIbB9MuZuAQJYrxRou0uq5cXpx2pH?usp=sharing}{Google Colab} no formato \textit{Jupyter Notebook} e no repositório \href{https://github.com/MatMB115/TFG-UNIFEI-scope-review-about-deepfakes-detection}{Revisão de Escopo da Literatura Sobre Detecção de Deepfake} hospedado pelo \textit{Github}.

==> elempostextuais/apenB.tex <==
\chapter{Título do Apêndice B}
\label{apendiceB}

Edite o arquivo ``\textcolor{magenta}{\textit{elempostextuais > apen2.tex''}}.

==> elempretextuais/abreviaturas.tex <==
% - Descreva abaixo o acrônimo como \acro{acrônimo}{Descrição}
% - Utilize \ac{acrônimo} toda vez que for citar o acrônimo no texto. Na 1ª ocorrência é descrito o significado, nas demais o acrônimo contém o link para a lista de acrônimos.
% - É necessário colocá-los em ordem alfabética pois a ordenação não é feita automaticamente.
% Para evitar Warnings exclua da relação abaixo os acrônimos que não utilizou no texto.
%
\begin{acronym}[UNIFEI] % Coloque aqui o acrônimo mais longo para melhor alinhamento
    \acro{AE}{Autoencoder}
    \acro{AUC}{Area Under The Curve}
    \acro{CE}{Cross Entropy Loss}
    \acro{CNN}{Convolutional Neural Network}
    \acro{CPU}{Central Processing Unit}
    \acro{CUDA}{Compute Unified Device Architecture}
    \acro{DF}{Deepfake}
    \acro{DFDC}{DeepFake Detection Challenge}
    \acro{DFGC}{DeepFake Game Competition}
    \acro{DL}{Deep Learning}
    \acro{DNN}{Deep Neural Network}
    \acro{ED}{Encoder-Decoder}
    \acro{GAN}{Generative Adversarial Network}
    \acro{GenConViT}{Generative Convolutional Vision Transformer}
    \acro{GPU}{Graphics Processing Unit}
    \acro{GELU}{Gaussian Error Linear Unit}
    \acro{GRU}{Gated Recurrent Unit}
    \acro{HOG}{Histogram of Oriented Gradients}
    \acro{IA}{Inteligência Artificial}
    \acro{LSTM}{Long Short-Term Memory}
    \acro{ML}{Machine Learning}
    \acro{MLP}{Multilayer Perceptron}
    \acro{MSE}{Mean Squared Error}
    \acro{RAM}{Random Access Memory}
    \acro{ReLU}{Rectified Linear Unit}
    \acro{ROC}{Receiver Operating Characteristic}
    \acro{RGB}{Red, Green and Blue}
    \acro{RNA}{Redes Neurais Artificiais}
    \acro{RNN}{Recurrent Neural Network}
    \acro{SPSL}{Spatial-Phase Shallow Learning}
    \acro{SVM}{Support Vector Machine}
    \acro{UCF}{Uncovering Common Features}
    \acro{UNIFEI}{Universidade Federal de Itajubá}
    \acro{VAE}{Variational Autoencoder}
    \acro{vCPU}{Virtual Central Processing Unit}
    \acro{ViT}{Vision Transformers}
\end{acronym}

==> elempretextuais/abstract.tex <==
% Traducao do resumo para a lingua inglesa

The growing threat posed by deepfake videos, capable of manipulating realities and disseminating misinformation, drives the urgent need for effective detection methods. This work investigates and compares different approaches for identifying deepfakes, focusing on the GenConViT model and its performance relative to other architectures present in the DeepfakeBenchmark. To contextualize the research, the social and legal impacts of deepfakes are addressed, as well as the technical fundamentals of their creation and detection, including digital image processing, machine learning, and artificial neural networks, with emphasis on Convolutional Neural Networks (CNNs), Generative Adversarial Networks (GANs), and Transformers. The performance evaluation of the models was conducted using relevant metrics and new datasets established in the literature, such as WildDeepfake and DeepSpeak, aiming to identify the most effective tools in the battle against misinformation and media manipulation. The obtained results indicated that GenConViT, after fine-tuning, exhibited superior performance in terms of accuracy (93.82\%) and generalization capacity, surpassing other architectures in the DeepfakeBenchmark on the DeepSpeak dataset. This study contributes to the advancement of deepfake detection techniques, offering contributions to the development of more robust and effective solutions against the dissemination of false information.

==> elempretextuais/agradecimentos.tex <==
Agradeço primeiramente a meus pais, Isaac e Izabel, aos quais serei eternamente grato por tudo o que fizeram e fazem por mim, por todo o incentivo e suporte, pela ajuda em superar as dificuldades e por compartilhar as vitórias e os momentos de felicidade. Sem eles nada disso teria sido possível.

Agradeço também a todos os professores que me guiaram nessa jornada, desde os níveis mais básicos e fundamentais de minha educação, até o nível em que me encontro hoje. Obrigado!

Em especial, agradeço à minha orientadora, Profa. Dra. Isabela Drummond e meu primo Felipe, pela incrível paciência, pelos conselhos, pela compreensão e pelos ensinamentos ao decorrer deste trabalho, que não teria sido possível sem o norte que me proporcionaram. Obrigado!
Inspiro-me muito em vocês e espero que essa parceria se estenda por muitos anos.

Agradeço à minha companheira e namorada, Clara, por sempre estar ao meu lado, em todos os momentos, me incentivando, me dando apoio e carinho.

Agradeço também ao meu tio David e às minhas tias Maria do Carmo, Marialba e Meire por sempre possibilitarem e incentivarem meus estudos.

==> elempretextuais/epigrafe.tex <==
% Texto
\textit{A realidade é aquilo que, quando você para de acreditar, não desaparece.}

% Autor/Fonte
\textsc{Philip Kindred Dick}

==> elempretextuais/resumo.tex <==
% Resumo do trabalho em um unico paragrafo

A crescente ameaça representada pelos vídeos \textit{deepfake}, capazes de manipular realidades e disseminar desinformação, impulsiona a necessidade urgente por métodos eficazes de detecção. Este trabalho investiga e compara diferentes abordagens para a identificação de \textit{deepfakes}, com foco no modelo \textit{GenConViT} e sua performance em relação a outras arquiteturas presentes no \textit{DeepfakeBenchmark}. Para contextualizar a pesquisa, são abordados os impactos sociais e legais dos \textit{deepfakes}, além dos fundamentos técnicos de sua criação e detecção, incluindo processamento de imagens digitais, aprendizado de máquina e redes neurais artificiais, com destaque para as Redes Neurais Convolucionais (CNNs), Redes Generativas Adversárias (GANs) e \textit{Transformers}. A avaliação do desempenho dos modelos foi realizada utilizando métricas relevantes e conjuntos de dados novos estabelecidos na literatura, como \textit{WildDeepfake} e \textit{DeepSpeak}, visando identificar as ferramentas mais eficazes na luta contra a desinformação e manipulação da mídia. Os resultados obtidos indicaram que o \textit{GenConViT}, após ajuste fino, apresentou desempenho superior em termos de acurácia (93,82\%) e capacidade de generalização, superando outras arquiteturas no \textit{DeepfakeBenchmark} no conjunto \textit{DeepSpeak}. Este estudo contribui para o avanço das técnicas de detecção de \textit{deepfakes}, oferecendo contribuições para o desenvolvimento de soluções mais robustas e eficazes contra a disseminação de informações falsas.

==> elempretextuais/simbolos.tex <==
% Insira abaixo seus símbolos conforme o modelo:
% simbolo (separador: &~&) descricao (quebra de linha: \\)

$f(x, y)$ & Função de intensidade luminosa de uma imagem \\
$i(x, y)$ & Iluminância (quantidade de luz incidente) \\
$M \times N$ & Dimensões da matriz de uma imagem digital \\
$L$ & Número inteiro de níveis de quantização \\
$\mathcal{X}$ & Conjunto de dados de entrada \\
$\omega_i$ & Pesos associados ao \(i\)-ésimo sinal no Perceptron \\
$b$ & Valor de viés (bias) no Perceptron \\
$\chi_i$ & \(i\)-ésimos sinais de entrada do Perceptron \\
$\sigma(x)$ & Função Sigmoid \\
$\text{ReLU}(x)$ & Função de ativação ReLU (\textit{Rectified Linear Unit}) \\
$\text{GELU}(x)$ & Função de ativação GELU (\textit{Gaussian Error Linear Unit}) \\
$L_{CE}$ & Perda por Entropia Cruzada \\
$L_{MSE}$ & Erro Quadrático Médio (Mean Squared Error) \\
$L_{logv}$ & Erro de Reconstrução (Log-Verossimilhança) em VAE \\
$L_{KL}$ & Termo de perda da Divergência de Kullback-Leibler em VAE \\
$L_{recon}$ & Termo de perda de reconstrução em VAE \\
$L_{VAE}$ & Função de perda total em VAE \\
$\mu$ & Média da distribuição no espaço latente \\
$\sigma^2$ & Variância da distribuição no espaço latente \\
$\mathcal{N}(\mu, \sigma^2)$ & Distribuição normal com média \(\mu\) e variância \(\sigma^2\) \\
$z$ & Representação no espaço latente \\
$\epsilon$ & Ruído amostrado de uma distribuição \(\mathcal{N}(0, I)\) no truque de reparametrização \\
$(f * g)(k)$ & Convolução das funções \(f\) e \(g\) \\
$h(k)$ & Resultado da convolução \\
$f(i)$, $g(k-i)$ & Valores das sequências numéricas \(f\) e \(g\) \\
$k$ & Índice da sequência resultante da convolução \\
$f_{l+1}(i, x, y)$ & Pixel resultante da filtragem da imagem na camada anterior \(l\), processada pelo filtro \(i\) \\
$G(x)$ & Função Geradora (em GANs) \\
$D(x)$ & Função Discriminadora (em GANs) \\
$L_{adv}(D)$ & Função de perda adversarial para o Discriminador \\
$L_{adv}(G)$ & Função de perda adversarial para o Gerador \\
$x$ & Dados de entrada \\
$x'$ & Reconstrução dos dados de entrada \\
$x_s$, $x_t$ & Imagens que representam as identidades de origem e alvo, respectivamente \\
$x_g$ & Imagem gerada a partir das identidades de origem e alvo \\
$D_{KL}(q \| p)$ & Divergência de Kullback-Leibler entre duas distribuições \(q\) e \(p\) \\
$D_e(z)$ & Função do decodificador \\
$FP$ & Falsos Positivos \\
$FN$ & Falsos Negativos \\
$VP$ & Verdadeiros Positivos \\
$VN$ & Verdadeiros Negativos \\

